A General Approach to Approximate Multistage Subgraph Problems

In a Subgraph Problem we are given some graph and want to find a feasible subgraph that optimizes some measure. We consider Multistage Subgraph Problems (MSPs), where we are given a sequence of graph instances (stages) and are asked to find a sequence of subgraphs, one for each stage, such that each is optimal for its respective stage and the subgraphs for subsequent stages are as similar as possible. We present a framework that provides a $(1/\sqrt{2\chi})$-approximation algorithm for the $2$-stage restriction of an MSP if the similarity of subsequent solutions is measured as the intersection cardinality and said MSP is preficient, i.e., we can efficiently find a single-stage solution that prefers some given subset. The approximation factor is dependent on the instance's intertwinement $\chi$, a similarity measure for multistage graphs. We also show that for any MSP, independent of similarity measure and preficiency, given an exact or approximation algorithm for a constant number of stages, we can approximate the MSP for an unrestricted number of stages. Finally, we combine and apply these results and show that the above restrictions describe a very rich class of MSPs and that proving membership for this class is mostly straightforward. As examples, we explicitly state these proofs for natural multistage versions of Perfect Matching, Shortest s-t-Path, Minimum s-t-Cut and further classical problems on bipartite or planar graphs, namely Maximum Cut, Vertex Cover, Independent Set, and Biclique.

==> tikz-MMaxWBEC-hardness.tex <==
\begin{tikzpicture}[]
%	\useasboundingbox[green] (-4,-1.25) rectangle (4,1.25);
	\tikzset{dot/.style={draw,circle,fill=black,inner sep=1.5}}
	\tikzset{R/.style={superred,line width=.4mm}}
	\tikzset{B/.style={superblue,semithick,decorate,decoration={snake, segment length=2mm, amplitude=.5mm}}}
	\tikzset{dots/.style={B,semithick,densely dotted}}

	% vertex cycle X_v
	\node[dot] (Cx1) at (0,0) {};
	\node[dot] [above of=Cx1] (Cx2) {};
	\node[dot] [below left of=Cx1,yshift=3mm] (Cx0) {};
	\node[dot] [above left of=Cx2,yshift=-3mm] (Cx3) {};

	\draw (Cx0) edge[B] (Cx1);
	\draw (Cx1.center) edge[B] (Cx2.center);
	\draw (Cx2) edge[B] (Cx3);

	\node [left of=Cx3,xshift=4.5mm] (Cx5x) {};
	\node [left of=Cx3,xshift=2.5mm] (Cx5) {};
	\draw (Cx3.center) edge[dots] (Cx5);
	\draw (Cx3.center) edge[B] (Cx5x);
	\node [left of=Cx0,xshift=4.5mm] (Cx-1x) {};
	\node [left of=Cx0,xshift=2.5mm] (Cx-1) {};
	\draw (Cx0.center) edge[dots] (Cx-1);
	\draw (Cx0.center) edge[B] (Cx-1x);

	% edge cycle Y_{vw}

	% vertex cycle X_w
	\node[dot] (Cy1) at (3,0) {};
	\node[dot] [above of=Cy1] (Cy2) {};
	\node[dot] [below right of=Cy1,yshift=3mm] (Cy0) {};
	\node[dot] [above right of=Cy2,yshift=-3mm] (Cy3) {};

	\draw (Cy0) edge[B] (Cy1);
	\draw (Cy1.center) edge[B] (Cy2.center);
	\draw (Cy2) edge[B] (Cy3);

	\node [right of=Cy3,xshift=-4.5mm] (Cy5x) {};
	\node [right of=Cy3,xshift=-2.5mm] (Cy5) {};
	\draw (Cy3.center) edge[dots] (Cy5);
	\draw (Cy3.center) edge[B] (Cy5x);
	\node [right of=Cy0,xshift=-4.5mm] (Cy-1x) {};
	\node [right of=Cy0,xshift=-2.5mm] (Cy-1) {};
	\draw (Cy0.center) edge[dots] (Cy-1);
	\draw (Cy0.center) edge[B] (Cy-1x);


	\draw (Cx1.center) edge[R] (Cx2.center);
	\draw (Cx1.center) edge[R] (Cy1.center);
	\draw (Cy1.center) edge[R] (Cy2.center);
	\draw (Cx2.center) edge[R] (Cy2.center);

	\foreach \x in {0,...,3}{
		\node[dot] at (Cx\x) {};
		\node[dot] at (Cy\x) {};
	}
	\node[draw,circle,semithick,fill=none,minimum width=3mm,inner sep=0] at (Cx1) {};
	\node[draw,circle,semithick,fill=none,minimum width=3mm,inner sep=0] at (Cx3) {};
	\node[draw,circle,semithick,fill=none,minimum width=3mm,inner sep=0] at (Cy1) {};
	\node[draw,circle,semithick,fill=none,minimum width=3mm,inner sep=0] at (Cy3) {};
\end{tikzpicture}


==> tikz-sandwich.tex <==
\begin{tikzpicture}[xscale=1,transform shape]

	\draw [-latex](-0.5,0) coordinate(dd)-- (0,0) coordinate (O1) -- (17,0)coordinate(ff) node[above]{$t$};
	\draw [dashed,thick] (O1) -- (0,1) coordinate(S3) -- (0,3) coordinate(S2) -- (0,5) coordinate(e3) -- ++(0,1)coordinate(ff2);

	\foreach \nn in{S3,S2,e3}{
		\draw [thick] (dd|-\nn) node[above]{\nn}-- (\nn-|ff);
	}

	\foreach \xx in{1,2,...,16}{
		\draw[dashed] (\xx,0) -- (\xx,0|- ff2);
	}

	\foreach \xx in{0,4,8,...,16}{
		\draw[dashed] (\xx,0.2) -- (\xx,-0.2) node[below]{\xx 0};
	}

	\begin{scope}[shift={(e3)}]
		\node[ above right=0.4cm and 0cm of e3,right,draw, minimum width=4cm,minimum height=0.8cm,fill=white](n3a) {$3=f(e_3)$};
		\draw[-latex,thick] (n3a.north west) -- ++(0,0.5)node[right]{$a^{e3}_{3=f(e3)}$};
	\end{scope}

	\begin{scope}[shift={(S2)}]
		\coordinate(O2) at (2,0);
		\node[ above right=0.4cm and 0cm of O2,right,draw, minimum width=4cm,minimum height=0.8cm,fill=white](n4a) {$4=f(s_2)$};
		\draw[-latex,thick,green] (n4a.north west) -- ++(0,0.5)node[right,fill=white]{$a^{S2}_{f(S2)}$};
		\draw[-latex,thick,blue] ([xshift=2.7cm]n4a.north west) coordinate(bb1)-- ++(0,0.5)node[right,fill=white]{$a^{S2}_{3=f(e3)}$};
		\draw[dashed,red] (n3a.south east) -- (bb1);
		\node[right=0cm of n4a,right,draw, minimum width=4cm,minimum height=0.8cm,fill=white](n3b) {$3=p(e_3)$};
	\end{scope}

	\begin{scope}[shift={(S3)}]
		\coordinate(O3) at (0.5,0);
		\node[ above right=0.4cm and 0cm of O3,right,draw, minimum width=4cm,minimum height=0.8cm,fill=white](n1) {$1=f(s_2)$};
		\node[right=0cm of n1,right,draw, minimum width=4cm,minimum height=0.8cm,fill=white](n5) {$5$};
		\node[right=0cm of n5,right,draw, minimum width=4cm,minimum height=0.8cm,fill=white](n4b) {$4=p(S2)$};
		\node[right=0cm of n4b,right,draw, minimum width=4cm,minimum height=0.8cm,fill=white](n3c) {$3$};
	\end{scope}
\end{tikzpicture}

